The Atacama Cosmology Telescope: Data Characterization and Map Making

We present a description of the data reduction and mapmaking pipeline used for the 2008 observing season of the Atacama Cosmology Telescope (ACT). The data presented here at 148 GHz represent 12% of the 90 TB collected by ACT from 2007 to 2010. In 2008 we observed for 136 days, producing a total of 1423 hours of data (11 TB for the 148 GHz band only), with a daily average of 10.5 hours of observation. From these, 1085 hours were devoted to a 850 deg^2 stripe (11.2 hours by 9.1 deg) centered on a declination of -52.7 deg, while 175 hours were devoted to a 280 deg^2 stripe (4.5 hours by 4.8 deg) centered at the celestial equator. We discuss sources of statistical and systematic noise, calibration, telescope pointing, and data selection. Out of 1260 survey hours and 1024 detectors per array, 816 hours and 593 effective detectors remain after data selection for this frequency band, yielding a 38% survey efficiency. The total sensitivity in 2008, determined from the noise level between 5 Hz and 20 Hz in the time-ordered data stream (TOD), is 32 micro-Kelvin sqrt{s} in CMB units. Atmospheric brightness fluctuations constitute the main contaminant in the data and dominate the detector noise covariance at low frequencies in the TOD. The maps were made by solving the least-squares problem using the Preconditioned Conjugate Gradient method, incorporating the details of the detector and noise correlations. Cross-correlation with WMAP sky maps, as well as analysis from simulations, reveal that our maps are unbiased at multipoles ell > 300. This paper accompanies the public release of the 148 GHz southern stripe maps from 2008. The techniques described here will be applied to future maps and data releases.

==> pre-processing.tex <==
\section{Pre-processing}
\label{pre-processing}
In addition to data selection, calibration and pointing, there are a few other pre-processing steps that are done to the data before solving for the maps, or used for characterizing systematics.
Here we discuss these steps and provide some insight into their effects on the data.

\subsection{Downsampling}

As described in Section~\ref{signals}, the celestial signal bandwidth (nearly $30\,\hertz$) is significantly lower than the data bandwidth, the latter of which is $200\,\hertz$ given our $400\,\hertz$ sample rate.
This means that the data can be downsampled by a factor of two without losing significant information, while reducing both the memory required and computational burden for data processing.

Before downsampling, the data are low-pass filtered using a time-domain triangular kernel of the form [0.25, 0.50, 0.25], which reduces the power by a factor of 4 at the new Nyquist frequency.
If the signal were white, the aliased noise from downsampling would increase the TOD rms~by a factor $\sqrt{8/3}$ when using the previous filter.
This noise increase takes place mostly at the high end for the TOD spectrum, so the signal band remains almost unaffected.

\subsection{Anti-alias Filter and Optical Time-constant De-convolution}

To minimize aliasing when sampling the detectors, the data are filtered at the readout stage as discussed in Section \ref{random_noise}. 
To reverse the effect of the filter within the signal bandwidth, the inverse filter is applied during the pre-processing stage for map-making.

Similarly, the detector's optical time constants effectively filter the data as a single-pole low-pass filter.
We compensate their effect by applying the corresponding inverse filter to the data before map-making.

%\subsection{High-pass filter at $0.5\,\hertz$}
%We de-weight the data below $0.5\,\hertz$ using a sine squared filter with equation
%\begin{equation}
%G\left(f\right) = \left\{ \begin{array}{cl} 0 & {|f|\leq f_c-\frac{f_\Delta}{2}}\\ 
%\sin^2\left[\frac{\pi}{2}\left(\frac{|f| - f_c}{f_\Delta} + \frac{1}{2}\right)\right] & f_c-\frac{f_\Delta}{2} < |f| \leq f_c + \frac{f_\Delta}{2}\\ 
%1 & f_c + \frac{f_\Delta}{2} < |f| \end{array} \right.,
%\end{equation}
%where $f_c$ is the frequency at which the filter gain is $0.5$, and $f_\Delta = 0.1\,\hertz$ is the frequency gap that takes the filter to go from zero to one. 

%High-pass filtering the data helps to remove the strong atmosphere and temperature drifts, reducing the large-scale noise and stripping. It also highly depresses the CMB signal below l = 300. 

\subsection{Mode Selection and Removal}
\label{mode_removal}

Contaminant signals, like the atmosphere and systematic signals, produce correlations between detector TODs.
This can be modeled as a common time-stream (the contaminant signal) superimposed on the data in a set of individual detectors.
We call this time-stream a ``correlated mode''.
One way to estimate it is by representing it with an appropriate linear combination of detector TODs. 
For instance, the common mode, defined as a linear combination with equal weight of all detector TODs, is a good estimator of the atmosphere signal.
Organizing all the detector TODs into columns of an $n_{sample}$ by $n_{detector}$ matrix $\mathbf{A}$, this can be expressed as 

\begin{equation}
\mathbf{\hat{m}} = \mathbf{A}\mathbf{\hat{v}}s^{-1},
\label{linear_comb}
\end{equation}

\noindent where $\mathbf{\hat{v}}$ is a vector of unit magnitude representing the $n_{detector}$ coefficients of the linear combination, and $s$ normalizes the mode so it also has unit magnitude.
To simplify the notation, we henceforth define the correlated modes such that they are always normalized.

Once a correlated mode has been identified, it can be fit and subtracted from the data:

\begin{equation}
\label{de-projection}
\mathbf{A}' = \left(\mathbf{I} - \mathbf{\hat{m}\hat{m}}^T\right) \mathbf{A} =
              \mathbf{A}\left(\mathbf{I} - 
              \mathbf{\hat{v}\hat{v}}^T\mathbf{A}^T\mathbf{A}\,s^{-2}\right), 
\end{equation}

\noindent where the last equality only holds when the mode is an actual linear combination of the data defined by $\mathbf{\hat{v}}$. 
For instance, one could obtain $\mathbf{\hat{m}}$ from a combination of dark detector TODs or from any other external source, like for example a thermometry time-stream. 

One can identify important correlated modes using the singular value decomposition (SVD) of the matrix $\mathbf{A}$:
\begin{equation}
\mat{A} = \mat{U}\,\mat{S}\,\mat{V}^T,
\end{equation}
where the columns of $\mat{U}$ can be identified as normalized correlated modes $\mathbf{\hat{m}}$, $\mat{S}$ is a diagonal matrix containing the singular values of $\mat{A}$ (identified as the normalization factor, $s$, in Equation \ref{linear_comb}), and the columns of $\mat{V}$ are the eigenvectors of the covariance matrix $\mat{A}^T\mat{A}$ (identified as vector $\mathbf{\hat{v}}$ in Equation \ref{linear_comb}).
The SVD mode selection can be improved by forcing an arbitrary prior on the linear combination of TODs. 
For example, to find modes that are more likely to correlate in rows, we first find the common mode from all detector TODs in each row (32 row common modes in total), and stack them together as columns of a matrix $\mathbf{A}_{row}$.
The strongest modes are then readily found using SVD.
This method is useful to identify column correlated modes and sub-array scale modes from the atmosphere. 
For the latter, we divide the array into 16 square blocks, finding the common mode in each one before applying the SVD. 
We call the set of modes found this way a ``multi-common mode.''

\subsubsection{Mode Removal Effects on the Celestial Signal}

An important consideration when using modes obtained from linear combinations of live detectors is that they are also correlated to the sky signal.
For example, naively removing the common mode effectively filters the sky, depressing scales larger than the array size ($\approx\!24\arcmin$ or $\ell\lesssim450$).
Naturally, the effect is stronger for the multi-common mode, which filters scales larger than a forth of the array ($\approx\!6\arcmin$ or $\ell\lesssim1800$).
For this reason, the multi-common mode is used to calculate the drift error, but it cannot be naively removed for making maps, nor can any other mode obtained from live detectors.

In Section~\ref{map-making}, the appropriate way of projecting modes out of the data is discussed in the context of map-making.

\subsubsection{Dark Mode Removal}

The dark detectors share the same readout as the live detectors, so they can capture systematics like thermal drift, electromagnetic pickup and magnetic pickup.
Moreover, as they are not coupled to the optical signal, correlated modes obtained from dark detectors (dark modes) can be safely removed as a preprocessing step before making maps.

The thermal drift is well-represented by the low-pass filtered common mode of the dark detectors.

For row- and column-correlated electromagnetic signals, the ability to identify correlated modes depends on whether there is a working dark detector in the desired row or column of the array.
By design there is one dark detector per column, always in the same row.
This is ideal for identifying column correlated modes, but not for row correlated modes.
For the latter we must rely on the broken live detectors with properly working readout circuit, as described in Section \ref{data_selection}.
Nevertheless, the row and column correlated modes can still be identified by using SVD analysis over all dark detectors.\footnote{It is useful to first remove the slow thermal drift from the dark detectors before trying to find these other higher frequency signals.} 
Figure \ref{sync_Mcm_corr} shows an example of correlation matrices before and after having removed the dark modes.
Note that both column and row correlations have been significantly suppressed.

